Towards Virtual Clinical Trials of Radiology AI with Conditional Generative Modeling

Artificial intelligence (AI) is poised to transform healthcare by enabling personalized and efficient care through data-driven insights. Although radiology is at the forefront of AI adoption, in practice, the potential of AI models is often overshadowed by severe failures to generalize: AI models can have performance degradation of up to 20% when transitioning from controlled test environments to clinical use by radiologists. This mismatch raises concerns that radiologists will be misled by incorrect AI predictions in practice and/or grow to distrust AI, rendering these promising technologies practically ineffectual. Exhaustive clinical trials of AI models on abundant and diverse data is thus critical to anticipate AI model degradation when encountering varied data samples. Achieving these goals, however, is challenging due to the high costs of collecting diverse data samples and corresponding annotations. To overcome these limitations, we introduce a novel conditional generative AI model designed for virtual clinical trials (VCTs) of radiology AI, capable of realistically synthesizing full-body CT images of patients with specified attributes. By learning the joint distribution of images and anatomical structures, our model enables precise replication of real-world patient populations with unprecedented detail at this scale. We demonstrate meaningful evaluation of radiology AI models through VCTs powered by our synthetic CT study populations, revealing model degradation and facilitating algorithmic auditing for bias-inducing data attributes. Our generative AI approach to VCTs is a promising avenue towards a scalable solution to assess model robustness, mitigate biases, and safeguard patient care by enabling simpler testing and evaluation of AI models in any desired range of diverse patient populations.

==> old_material/2024-10-01_intro.tex <==

% Vendors can use patient attributes, such as sex, age, height, and weight, to condition image generation, since they are more easily collected or modeled based on real populations, even those with no existing image data.
% However, synthesizing full virtual patients poses significant challenges.
% It is necessary to maintain global consistency with conditioning attributes as well as anatomical correctness over the full body, but volumetric image synthesis of full patients is memory intensive.


% Conditional image synthesis is defined by the ability to generate realistic images from a specific patient cohort, enabling \emph{in silico} imaging trials of AI algorithms that estimate their performance in real clinical trials on the same population (Fig.~\ref{fig:overview-synth}).
% This is an invaluable capability for institutions looking to adopt the latest advances in precision medicine, for regulators aiming to standardize approval pipelines for AI, as well as for researchers seeking to improve their algorithms.
% Before purchasing an AI-equipped imaging system, for instance, an institution could generate synthetic images based on its own medical records, conducting an \emph{in silico} trial of the new system that informs the purchasing decision and allows the institution to anticipate its effect on current practice. On the other end of the development cycle, researchers can use \emph{in silico} imaging trials to identify algorithmic vulnerabilities, for instance because a crucial sub-population is under-represented in the training set, thereby avoiding failed submissions to regulators or patient-facing failures after deployment. Armed with detailed knowledge about which combinations of patient attributes lead to deteriorated performance, researchers can augment real training data with synthetic images in a targeted manner to rectify the imbalance and drive forward ongoing development.

% It's an unsolved problem: People have tried to do this. How broad do we want to go here? Let's structure a little bit. We are discussing conditioning image generation on attributes to facilitate algorithm validation. There are two pieces there: realistic CT synthesis and medical algorithm validation with synthetic data. Let's take those in order, starting with validating algorithms with synthetic data, which is likely to be the first sticking point.
% We do want to look at medical image synthesis for training AI algorithms, so that we can cite DeepDRR, SyntheX, and all our other
% Mathias: We don't want it to seem like this has been done before at all. Yes, medical image synthesis has been used for this purpose before, but what's the novelty? What's new in this approach?
% Conditional image synthesis represents a major step forward in the use of synthetic medical images for evaluating AI algorithm performance.

% Until now, synthetic medical image generation has lacked the combination of realism and control that is necessary for \emph{in silico} imaging trials of AI algorithms.
% One prominent source of synthetic medical images are virtual patient phantoms, which range from stylized combinations of geometric primitives to statistical atlases based on patient populations.\cite{peng2022review, abadi2020virtual} In combination with physics-based imaging simulations, these can be used to synthesize medical images from various imaging modalities,\cite{killeen2023insilico, abadi2020virtual} including CT,\cite{segars2008realistic, badal2009accelerating, maier2013conrad} MRI,\cite{buoso2023mrxcat} PET and SPECT,\cite{herraiz2024mcgpu} ultrasound, mammography,\cite{aldo2018evaluation, badal2021mammography} and X-ray.\cite{unberathopen} A major limitation of virtual patient phantoms is the lack of intra-organ heterogeneous details,\cite{amirrajab2020xcat} leading to various strategies for texturing or otherwise adding detail to virtual phantoms and simulated images.\cite{abadi2020virtual} This can be done through proceduraly generated textures\cite{bakic2003mammogram} or disease models\cite{hoe2006simulation, zhang2007simulating} on a per-organ basis, or through image-to-image translation models using deep learning.\cite{chang2020development, amirrajab2020xcat} While virtual patient phantoms have enabled \emph{in silico} trials of AI algorithms,\cite{lowther2018investigation, tushar2022virtual} they \todo{fundamentally represent an untethering of patient-based image characteristics from the attributes used for conditioning.}

% Broadly, machine learning-based methods for CT image synthesis have been gradually maturing. They include image-to-image translation models for bringing phantom,\cite{tushar2022virtual} MR,\cite{han2017mr, lei2019mri, pan2023synthetic, bahrami2021comparison} and CBCT\cite{chen2020synthetic, peng2024cbct, fu2024energy} images into the patient CT domain, which can augment existing data for training downstream algorithms. Purely generative models have also been proposed,\cite{sorin2020creating} which can be conditioned on attributes like disease presence.\cite{jiang2020covid} Denoising diffusion probabilistic models\cite{ho2020denoising} significantly advanced the quality of CT image synthesis over previous generative models,\cite{khader2023denoising, txurio20203diffusion, pan20232d} enabling fine-grained control based on organ segmentations.\cite{konz2024anatomically} When combined with statistical shape models to produce these segmentations, such models can in theory provide a pathway toward conditional image synthesis for \emph{in silico} trials on unseen populations. However, they \todo{still represent a fundamental decoupling of the attributes used to condition images, which are available from medical records, and the visually and anatomically realistic images ultimately generated.}
% We contend that the ability to finely control the attributes of generated data, including properties which can only be confirmed by generating full-body images, is the next step in transitioning synthetic data from an augmentation to training data pipelines, which are ultimately tested on real data, to being a realistic testbed for algorithm performance that reflects real populations.

% Virtual patient phantoms, which can be voxelized to create CT images from a range of desired attributes, have provided researchers with data to ``quantitatively evaluate and improve imaging instrumentation, data acquisition, techniques, and image reconstruction and processing methods which can lead to improved image quality and more accurate clinical dianosis.''\cite{segars2008realistic} They range from stylized phantoms handcrafted from geometric primitives to realistic deformable atlases with finely controllable attributes.\cite{peng2022review}
% The XCAT phantoms, for example, have been used to forecast algorithm performance for COVID-19 diagnosis from chest CTs, correctly predicting failures when evaluated outside the source institution.\cite{tushar2022virtual}
% They have also been used for validating cardiac MRI tracking algorithms,\cite{lowther2018investigation} and they can be made more realistic using image-to-image generative models.\cite{amirrajab2020xcat}
% However, a major limitation of the XCAT phantoms, as well as other phantoms based on deformable shape atlases, is ``the lack of intra-organ anatomical details and textures,'' since all organs are defined as homogeneous materials within their respective surface shape models.\cite{amirrajab2020xcat}

% Crucially, this paper from Duke did not show that the virtual phantoms reproduce good results from the model, and they don't allow you to model populations in a randomized way that reflects real distributions, only different imaging zmodality-level choices.
% Much of the related work exploring generative AI for medical image synthesis focuses on augmenting training data for downstream algorithms, which are then evaluated on real data.\cite{chen2022generative}
% \todo{Review methods for CT/MRI generative modeling here, but emphasize that no one is using these to evaluate algorithm failure due to population shift}
% Medical image synthesis can be an effective data source for evaluating AI algorithm performance. \dots Medical image synthesis has also been used as an effective alternative to real data collection for training downstream algorithms. (simulation vs generative modeling)
% Then we look at augmenting/replacing training data with synthetic images?
% Medical image synthesis has played a prominent role in AI training and testing, ranging from the generation of  been proposed as an alternative to real data collection for the purpose of training algorithms. \todo{background on such models, SyntheX, GANs, diffusion, etc.}

% \section{A Full-body Generative Model for \textit{In Silico} CT Imaging Trials}

% % Here's our solution: both a model and a demonstration, in a precisely controlled setting, that full-body image synthesis can serve this purpose.
% The key capability introduced in this work is the generation of realistic, full-body CT images conditioned on high-level attributes, including sex, age, height, and weight. These attributes are easier to obtain than medical images, since they are routinely recorded during primary care and can be deidentified more easily than images. Even if they are not available, they can often be estimated based on public health data, \eg. the census. Using these attributes as a conditioning signal, we train a latent denoising diffusion model with a stacked VQ-GAN autoencoder backbone. \todo{more description of model}
% Our results find that these images are realistic in terms of both appearance and anatomy, comparable to other state-of-the-art CT image synthesis models. At the same time, because the generated images are full-body, their alignment with the conditioning attributes of sex, height, and weight can be directly verified. The alignment with respect to age can be estimated based on distributions of estimated bone density, which declines over time. On its own, this is a valuable capability for creating synthetic patient models in a finely controlled manner.

% For conducting \emph{in silico} imaging trials, the key question is whether conditioning on high-level patient attributes can generate synthetic image datasets that allow downstream algorithms to perform similarly to how they would on the corresponding real data. Can we anticipate real-world algorithm failures before they happen by testing on synthetic datasets? Using the aforementioned conditional model, we generate synthetic patient cohorts for evaluating downstream algorithms for body composition measurement, an important task for tailoring interventions to patients' unique metabolic profiles, which can differ markedly even among individuals with the same age, height, and weight.\cite{lemos2017current}

% \newpage

% % It's an interesting problem:
% In the emerging ecosystem of precision healthcare, access to medical image datasets from specific patient cohorts is crucial for developing and validating machine learning and artificial intelligence (ML/AI) algorithms. These algorithms can improve medical decision making \cite{ozsahin2020review, murugesan2022a, mohammadi2024deep} and support opportunistic disease screening \cite{pickhardt2013opportunistic, jang2019opportunistic,eng2021automated, oh2024evaluation}, but they rely on large scale image datasets with corresponding annotations for training, such as organ segmentation maps or disease indicators. Medical data are often difficult to obtain with sufficient quality and volume for training, due to the cost of collection and annotation.
% Moreover, medical datasets exhibit institution- or device-specific attributes, such as patient demographics or imaging protocol.
% Recent research on AI/ML model auditing has demonstrated fairness/bias concerns~\cite{Gichoya2022ReadingRace, Seyyed-Kalantari2021-aj, Seyyed-Kalantari2021-fa, Glocker2022-st, Henry_Hinnefeld2018-vi,pavlak2023data, beheshtian2022generalizability, bachina2023coarse, garin2023medical, morcos2023applying, li2023sex}, shortcut learning~\cite{winkler2019association, winkler2021association, nauta2021uncovering, jabbour2020deep, degrave2021ai,pavlak2023data, yi2022deep}, and lack of generalization or robustness~\cite{o2022evaluating,pavlak2023data, santomartino2024evaluating}.
% \emph{These failure modes are fundamentally similar}, because DNN performance deteriorates significantly when applied to sample distributions outside the training domain.
% The ability to finely control patient cohort sampling, therefore, would be invaluable for ensuring adequate representation of all relevant attributes in a dataset for ML/AI applications, firstly as a data source for training robust models and second, for evaluating model robustness on unseen populations.

% % Here's a more specific problem, which solves the above: gen AI-based cohort sampling, and it's an unsolved problem.
% \textbf{Synthetic cohorts} are collections of virtual patient models sampled from a desired distribution that support medical image generation. They provide realistic synthetic data without ethical restrictions \cite{khorchani2022sasc, pan20232d, txurio2023diffusion, khader2023denoising, cho2024medisyn}, and can support a range of annotations and specified attributes, including organ segmentations \cite{konz2024anatomically} and disease presence \cite{toda2021synthetic, jiang2020covid, zingarinim3dsynth}. Early works on learning-based medical image synthesis leveraged generative adversarial networks (GANs)~\cite{goodfellow2014generative} and CycleGANs~\cite{zhu2017unpaired} to augment existing data during the training process \cite{toda2021synthetic, han2017mr, lei2019mri}. With the advent of generative diffusion models \cite{ho2020denoising, rombach2022high}, these efforts have matured in terms of realism and capability \cite{kazerouni2023diffusion, ho2020denoising, rombach2022high, esser2020taming}, raising the possibility of fully sythetic cohorts for many applications that would otherwise require real data. However, existing generative medical image models are so far constrained in terms of supported anatomy \cite{khader2023denoising}, dimension \cite{txurio2023diffusion}, or conditioning capabilities \cite{2024addressing}. Txurio  \etal~\cite{txurio2023diffusion} first demonstrated that diffusion probabilistic models were a more viable approach to medical image synthesis than GANs, as measured in terms of the Frechet Inception Distance (FID) for CT image slices. Further work expanded diffusion-based models to 3D by conditioning image generation on adjacent slices \cite{han2023medgen3d, cho2024medisyn} or using 3D convolutions, conditioned on segmentation \cite{dorjsembe2023conditional, jiang2023cola, zingarinim3dsynth}. In one sense, conditioning on 3D segmentations is a desirable capability, because it enables tight control over models' generative process. On the other, it requires valid anatomical segmentations either from real images or from a statistical model based on real images, \eg. \cite{segars2018application}. This is an extra step that may be undesirable when there are no such data available from the desired cohort.

% % Here's our solution
% \emph{Our goal is to support synthetic patient cohorts of high-quality, full-body CT images and organ segmentations, conditioned on desired patient characteristics.}
% Existing approaches in this area focus on specific anatomical regions, such as the brain or abdomen \tocite{}, which are appropriate for specific downstream tasks. There is, however, an unmet need for full-body medical image synthesis, which can support imaging studies and downstream applications on varied anatomy as well as the whole body.
% Conditioning image generation on desired patient characteristics is necessary in order to support synthetic patient cohort generation directly.
% In this work, we focus on demographic characteristics, including sex, height, weight, age, and race, which are routinely included in electronic medical records.
% Using a dataset of \todo{798} full-body CT scans and meta-data from the New Mexico Descedent Image Database (NMDID) \cite{edgar2020new}, we propose a novel 3D denoising diffusion architecture capable of generating CT images conditioned on specific patient characteristics, using classifier-free conditioning on a latent representation of the full body. These images are sufficiently realistic to support multi-organ segmentation by TotalSegmentator~\cite{wasserthal2023totalsegmentator}, a multi-organ segmentation model trained on real images, and they can be generated \emph{ex nihilo}, \ie without any input images or segmentations, so as to support highly scalable cohort sampling.

% Our proposed model, contends directly with several unique challenges of conditional full-body CT image synthesis. The most immediate challenge is how to contend with the significant memory requirements for processing full-body CT images while maintaining global consistency. Rather than processing individual slices, we first encode 3D image patches using a stack of vector quantized generative adversarial networks (VQ-GAN) with a total $16\times$ compression. These patchwise latent codes are concatenated to form a full body latent space, on which a 3D-UNet-based diffusion network can be trained. In training the decoder, we introduce a novel dual-contrast reconstruction loss that ensures low-contrast soft tissue structure receive as much weight during training as high-contrast bony structures. To ensure the anatomical validity of sampled images, we train an additional VQ-GAN to represent a reduced segmentation map, thereby enabling our network to sample from the latent \emph{joint distribution} of CT and segmentations. Thus, our network generates a segmentation to go alongside each CT, and we further demonstrate that this step enables successful, independent segmentation by TotalSegmentator~\cite{wasserthal2023totalsegmentator}. \todo{We further compare our work to existing methods in terms of image realism.}

% To enable synthetic cohort generation, we train our model to support classifier-free conditioning based on demographic characteristics, following \cite{ho2022classifier}. Using the meta-data included in the NMDID dataset, we support specification of patient sex, height, weight, weight, age, and race. However, because NMDID is heavily biased toward older, white populations, we focus our evaluation primarily on the empirically verifiable properties of sex, height, and weight, evaluating whether synthetic CTs generated with TotalSynthesizer align with the desired distribution based on TotalSegmentator-derived metrics, such as the presence of sex organs or the weight as calculated based on an organ-specific density map computed from TotalSegmentator.


% Challenges we faced and how we deal with them
% - Not conditioning on the segmentation means global anatomical structure is difficult.
% - Full-body 3D images are big.
% - Soft tissue structures are low-contrast.
% -

% It's an unsolved problem: The txurio method is 2d only and not conditioned.
%
% Txurio is 2D only
% medisyn is text-conditioned, uses a latent diffusion model, with a 3D unet VAE. Limited in terms of resolution and size.
% Zingarinim injects desired perturbations into existing

% \todo{\cite{eng2021artificial}}

% Rather than collecting images retrospectively from a real-world institution,
% They are attractive as an alternative to real data collection, circumventing ethical and logistical constraints of working with patient data, and can provide certain annotations for ``free,'' depending on the representational power of the underlying algorithm. Recently, generative AI models have been used for conditional medical image synthesis, \eg. based on text descriptions \todo{cite}, that would enable large scale sampling from synthetic patient cohorts of chest X-rays \cite{} and histopathology slides \cite{}.
% \todo{Discuss the limited research into CT/MRI synthesis, and how it falls short in generating full body samples}


% % conclude second paragraph with this.
% The goal of this paper is to generate high quality full-body CT images and organ segmentations from synthetic patient cohorts using conditional generative models.


% % It's an unsolved problem: need to be able to condition full-body generation based on desired attributes, generating CTs with corresponding multi-organ segmentations.
% Generative modeling of medical images has received increasing attention as the associated algorithms and computational resources have matured \cite{kazerouni2023diffusion, kebaili20243d, txurio2023diffusion, cho2024medisyn, zingarinim3dsynth, dorjsembe2023conditional, han2023medgen3d, jiang2023cola}.

% \subsection{Related Work}
% \label{sec:related-work}

% \paragraph{Validation of medical image analysis algorithms}
% Bringing AI into clinical practice.

% \citep{kanbar2022implementation} discusses bringing AI algorithms into clinical practice: where are we now and what's needed in the future. Yeah, but mostly about NLP, so this isn't that useful.

% \citep{ramwala2024establishing}

% \paragraph{Image translation}
% A large body of work has considered CT image synthesis via image-to-image translation.

% % MRI to CT
% \cite{han2017mr} goes from MRI to CT using U-Net architecture, for registration and DRR methods.

% \cite{lei2019mri} uses CycleGANs to synthesize CTs based on MRI, allowing MRI to be used for dose calculation in radiotherapy.

% \cite{bahrami2021comparison} MR to CT translation review

% \cite{pan2024synthetic} MR to CT using 3D diffusion

% % CBCT to CT
% \cite{chen2020synthetic} goes from CBCT to CT, so that algorithms trained on CT can be used intra-operatively, using a U-Net architecture

% \cite{peng2024cbct} CBCT to CT, using denoising diffusion models to enable organ segmentation and dose calculation during radiotherapy.

% \cite{fu2024energy} CBCT to CT using energy-guided diffusion models

% % Review of sCT in radiotherapy
% \cite{spadea2021deep} reviews sCT for radiotherapy applications

% % Adding contrast, conditional
% \cite{kim2018contrast} generates contrast-enhanced CT from PET/CT images, using a conditional GAN.

% \paragraph{Medical Image Synthesis}
% \cite{jiang2020covid} generates CT images with a conditional GAN that have COVID-19

% \cite{pan20232d} uses a diffusion model with a Swin-transformer backbone to create 2D chest X-rays, heart MRI slices, pelvic CT slices, and abodmen CT slices, evaluated in terms of authenticity, quality, and diversity using Turing assessments conducted by 3 medical physicists.

% \cite{sorin2020creating} systematic review in this area.

% % Using Diffusion
% \cite{konz2024anatomically} controlling the anatomy of the generated images using segmentation-guided diffusion

% \cite{txurio2023diffusion} uses diffusion models to generate abdominal CT images, but only in 2D, and evaluate in terms of Frechet Inception Distance

% \cite{khader2023denoising} using 3D diffusion models to synthesize MRi and CT images, quantitatively evaluated by two radiologists in terms of ``realistic image appearance,'' ``anatomical correctness,'' and ``consistency between slices.'' Also demonstrates value for downstream task, for breast segmentation models.


% Then talk about what we've done.
Our framework aims to support virtual clinical trials of AI models in precision medicine.
We therefore introduce a single model for conditional CT image synthesis that is \begin{inlistalpha}
  \item\label{itm:real} realistic,
  \item\label{itm:full} full-body, and
  \item\label{itm:cond} conditioned on high-level patient attributes.
\end{inlistalpha}.
Image realism \ref{itm:real} ensures that observed changes in model performance are due. to the modeled population shifts and not any domain gap between the real and the synthetic. It consists of both low-level visual fidelity, as measured by perceptual metrics such as the Frechet Inception Distance (FID), and high-level anatomical consistency, as measured by a multi-organ segmentation model trained on real images, \ie, TotalSegmentator\cite{wasserthal2023totalsegmentator}.
Given that, the ability to synthesize volumetric, full-body images \ref{itm:full} guarantees that the generative model itself does not become a black box.
Using independent segmentations of the synthesized images, patient-specific measurements of the output image enable independent verification of the generative model's fidelity to conditioning parameters, such as height and weight (see Section~\ref{sec:alignment}).
Additional quantities important for precision medicine, such as body fat percentage, muscle mass, average bone density, \etc, can be estimated directly from the image and independent segmentation (see Section~\ref{sec:body-measures}).
Synthesizing full-body images is challenging, though, due to the memory utilization of generative ML models\cite{guo2024maisi} and the need for anatomical consistency over the full image.\cite{hamamci2023generatect}
Important related work addresses this issue by conditioning generation of a CT image $\mathbf{x}$ on a multi-organ segmentation $\mathbf{y}$,\cite{guo2024maisi} such as can be obtained from a virtual patient phantom.\cite{abadi2020virtual} This reduces the complexity of the learning problem since $P(\mathbf{x}|\mathbf{y})$ is constrained by the detailed organ segmentation. To support more flexible sampling, though, we set out to learn the joint distribution $P(\mathbf{x},\mathbf{y}|\mathbf{a})$, where $\mathbf{a}$ describes patient attributes (sex, age, height, and weight), while still ensuring anatomical consistency with $\mathbf{y}$.
This is accomplished through a latent diffusion model with stacked auto-encoders, a novel loss function for CT image synthesis, and off-classifier conditioning.
Separate encoders and decoders are trained for CT images and segmentations, with the diffusion model learning the joint distribution.
% The model is validated in terms of its visual realism in comparison with state-of-the-art methods trained on far more data; its anatomical consistency based on third-party segmentation of the CT image alone; and fidelity to the conditioning signal.
Finally, we demonstrate the value of this generative model for detecting changes in performance in AI models, using two tasks in precision medicine where a simulated population shift resulted in performance degradation.


==> old_material/2024-10-06_model_description.tex <==
The image autoencoder is a vector quantized variational auto-encoder (VQ-VAE) that operates on 3D image patches. To enable a high compression rate without sacrificing reconstruction quality,\cite{esser2020taming} we propose a stacked encoder-decoder design with low compression at each level but a high overall compression rate, as in Fig.~\ref{fig:architecture}a. Given a full-body CT image $\mathbf{X} \in \R^{H \times W \times D}$, let
\begin{equation}
  \label{eq:7}
  \mathbf{Z}_{\rm img} = \mathcal{E}_{\rm img}(\mathbf{X}) \text{~~~and~~~}
  \hat{\mathbf{X}} = \mathcal{D}_{\rm img}(\mathbf{Z}_{\mathrm{img}})
\end{equation} denote the patch-wise embedding and reconstruction, respectively, of the full-body image. The embedding $\mathbf{Z}_{\rm img}\in \R^{\frac{H}{16} \times \frac{W}{16} \times \frac{D}{16} \times E}$ consists of discrete codes downsampled by the cumulated compression rate, 16, with embedding dimension $E$.
The encoder $\mathcal{E}_{\rm img}$ and decoder $\mathcal{D}_{\rm img}$ use the architecture described in van den Oord \etal\cite{van2017neural} to perform vector quantization with $K$ codes, albeit with 3D convolutions instead of 2D. The final decoder uses the perceptual reconstruction loss $\mathcal{L}_{\rm rec}$ and adversarial discriminator loss $\mathcal{L}_{GAN}$ in Esser.\etal\cite{esser2020taming} Additionally, a multi-window L1 loss is introduced to re-scale the image output so that the soft tissue reconstruction contributes more equally to the loss gradient than it would otherwise. For two scalar voxel values $x, \hat{x} \in \R$, let
\begin{equation}
  \label{eq:8}
  \mathcal{L}_{\rm mw}(x, \hat{x}) =
  \begin{cases}
    \lambda_{\rm soft} |x - \hat{x}| & \text{if } x < \text{HU}_{\rm soft}\\
    \lambda_{\rm hard} |x - \hat{x}| & \text{else},
  \end{cases}
\end{equation}
where $\text{HU}_{\rm soft}$ is chosen as the upper boundary of soft tissue density values. We find that using stacked autoencoders and $\mathcal{L}_{\rm mw}$ in place of the L1 loss improves the peak signal to noise ratio (PSNR) of the reconstruction from 29.08 to 31.06.
The multi-window reconstruction loss also improves the anatomical consistency of soft tissue structures during both reconstruction and sampling.

The segmentation autoencoder is trained in a similar manner to the image autoencoder, using a single VQ-VAE with the same overall compression rate.
Given the full-body segmentation $\mathbf{Y} \in \R^{H \times W \times D}$, let
\begin{equation}
  \label{eq:9}
  \mathbf{Z}_{\rm seg} = \mathcal{E}_{\rm seg}(\mathbf{X}) \text{~~~and~~~}
  \hat{\mathbf{Y}} = \mathcal{D}_{\rm seg}(\mathbf{Z}_{\mathrm{seg}})
\end{equation} denote the patch-wise embedding and reconstruction, respectively, of the full-body segmentation.

encoder $\mathcal{E}_{\rm seg}$ and decoder $\mathcal{D}_{\rm seg}$ are trained to convergence using the DICE loss as the primary reconstruction loss, with perceptual and adversarial discriminator losses as well.\cite{esser2020taming} After convergence, the embeddings $\mathbf{Z}_{\mathrm{seg}}$ are stored to disk.

$\mathbf{x}_i \in \R^{h \times w \times d}$ denote the $i$\textsuperscript{th} 3D image patch. We use an overall compression rate of 16, so the final patch embedding and reconstruction are
\begin{equation}
    \label{eq:6}
    \mathbf{z}_{\mathrm{img},i}^{(1)} = \mathcal{E}_{\rm img}^{(1)}(\mathbf{x})
  \text{~~~and~~~} \hat{\mathbf{x}}_i^{(1)} = \mathcal{D}_{\rm img}^{(1)}(\mathbf{z}_{\mathrm{img},i}^{(1)}).
\end{equation}

The image autoencoder is a vector quantized variational auto-encoder (VQVAE)\cite{van2017neural} that operates on 3D image patches.
To enable a high compression rate without sacrificing reconstruction quality,\cite{esser2020taming} we propose a stacked encoder-decoder design with low compression rates at each level but a high overall compression rate, as in Fig~\ref{fig:architecture}a.

Given a full-body CT image $\mathbf{X}$ in the training set, let $\mathbf{x}_i \in \R^{h \times w \times d}$ denote the $i$\textsuperscript{th} 3D image patch.
The first image patch embedding $\mathbf{z}_{\mathrm{img},i}^{(1)}$ and reconstruction $\hat{\mathbf{x}}_i^{(1)}$ are given by
\begin{align}
  \label{eq:2}
  \mathbf{z}_{\mathrm{img},i}^{(1)} = \mathcal{E}_{\rm img}^{(1)}(\mathbf{x})
  \text{~~~and~~~} \hat{\mathbf{x}}_i^{(1)} = \mathcal{D}_{\rm img}^{(1)}(\mathbf{z}_{\mathrm{img},i}^{(1)}).
\end{align}
The encoder $\mathcal{E}_{\rm img}^{(1)}$ and decoder $\mathcal{D}_{\rm img}^{(l)}$ use the architecture described in van den Oord \etal\cite{van2017neural} with 3D instead of 2D convolutions, as well as the perceptual reconstruction loss $\mathcal{L}_{\rm rec}$ and adversarial discriminator loss $\mathcal{L}_{GAN}$ in Esser \etal.\cite{esser2020taming}
Additionally, a multi-window L1 loss is introduced. This simple modification re-scales the image output so that the soft tissue reconstruction contributes more equally to the loss gradient---compared to hard tissue reconstruction---than it would otherwise. For two scalar voxel values $x, \hat{x} \in \R$, let
\begin{align}
  \label{eq:3}
  \mathcal{L}_{\rm mw}(x, \hat{x}) =
  \begin{cases}
    \lambda_{\rm soft} |x - \hat{x}| & \text{if } x < \text{HU}_{\rm soft}\\
    \lambda_{\rm hard} |x - \hat{x}| & \text{else}
  \end{cases},
\end{align} where $\text{HU}_{\rm soft}$ is chosen as the upper boundary of soft tissue density values. Then $\mathcal{L}_{\rm mw}(\mathbf{x}_i, \hat{\mathbf{x}}_i)$ is the average over the patch. These losses are summed and weighted as described in Section~\todo{sec}.
After training $\mathcal{E}_{\rm img}^{(1)}$ and $\mathcal{D}_{\rm img}^{(l)}$ to convergence, a second VQVAE $\left(\mathcal{E}_{\rm img}^{(2)}, \mathcal{D}_{\rm img}^{(2)}\right)$, is trained to reconstruct highly compressed feature embeddings $\mathbf{z}_{\mathrm{img},i}^{(2)}$. These have the same architecture but are trained using only mean-squared error (MSE) for the loss function. Additional VQVAE layers might be used for further compression, allowing for higher resolution images to be represented in our framework. After convergence, we denote the final composition of embeddings $\mathbf{z}_{\mathrm{img},i} = \mathcal{E}_{\rm img}(\mathbf{x}_i)$ and reconstructions $\hat{\mathbf{x}}_{i} = \mathcal{D}_{\rm img}(\mathbf{z}_{\mathrm{img},i})$.

To encourage anatomical consistency, we separately encode the full-body image segmentation $\mathbf{Y}$ in a patch-wise manner.
Similar to above, we denote the segmentation patch as $\mathbf{y}_i \in \R^{h \times w \times d \times C}$, where $C$ is the number of classes, and the encoder and decoder as
\begin{equation}
  \label{eq:5}
  \mathbf{z}_{\mathrm{seg}, i} = \mathcal{E}_{\rm seg}(\mathbf{x}_i) \text{~~~and~~~} \mathbf{y}_i = \mathcal{D}_{\rm seg}(\mathbf{z}_{\mathrm{seg}, i}).
\end{equation}
These are trained to convergence using DICE loss as the primary reconstruction loss, with perceptual and adversarial discriminator losses as well.\cite{esser2020taming} After convergence, the embeddings $\mathbf{z}_{\mathrm{seg},i}$ are stored to disk.


==> old_material/2024-10-09_table_backup.tex <==

\begin{sidewaystable}[h]
\ra{1.3}
\centering
\caption{Validation on Downstream Tasks for Differently Biased Cohorts (Shortcut Split)}
\label{tab:shortcut-results}
\begin{tabular}{@{}p{0.1em} l l rr rr rr rr@{}}
\toprule
\multicolumn{3}{@{}l}{\textbf{Downstream Task}} & \multicolumn{2}{c}{MAE} & \multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{R\textsuperscript{2} Score} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
& Sample & Source &\multicolumn{1}{l}{Value} & \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value} &\multicolumn{1}{r}{CI} \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Muscle Percentage (\%)}} \\ %& \multicolumn{8}{@{}l}{\textbf{8/30 Shortcut \wrt Weight / Sex}}\\
& IID & Real & 1.20 & [0.98, 1.44] & 3.49 & [2.92, 4.21] & 1.55 & [1.26, 1.83] & 0.87 & [0.79, 0.92] \\
&& Recon & 1.34 & [1.07, 1.54] & 3.81 & [3.33, 4.38] & 1.67 & [1.42, 1.94] & 0.84 & [0.75, 0.89] \\ % muscle real shortcut recon_sr data (prelim)
&& Synth & 1.71 & [1.44, 2.07] & 5.08 & [4.11, 6.21] & 2.18 & [1.72, 2.51] & 0.74 & [0.56, 0.83] \\
& Weighted & Real & 2.49 & [1.26, 4.65] & 7.39 & [3.08, 13.35] & 2.19 & [2.25, 9.88] & \multicolumn{2}{c}{---}\\
& OOD & Real & 6.18 & [5.36, 6.98] & 27.35 & [22.94, 31.69] & 6.90 & [6.15, 7.62] & -1.67 & [-2.67, -0.98] \\
& & Recon & 4.75 & [4.15, 5.32] & 18.90 & [15.74, 21.75] & 5.33 & [4.75, 5.93] & -0.70 & [-1.45, -0.19] \\  % muscle real shortcut ood recon_sr data (prelim)
& & Synth & 3.70 & [3.28, 4.29] & 13.85 & [12.08, 15.77] & 4.32 & [3.88, 4.76] & 0.06 & [-0.35, 0.32]\\
\multicolumn{3}{@{}l}{\textbf{Body Fat Percentage (\%)}} \\ % & \multicolumn{8}{@{}l}{\textbf{8/30 Shortcut \wrt Weight / Sex}} \\
& IID & Real & 1.24 & [1.00, 1.41] & 5.79 & [3.99, 7.37] & 1.61 & [1.31, 1.88] & 0.98 & [0.96, 0.98] \\
& & Recon & 1.23 & [0.97, 1.43] & 5.60 & [3.85, 7.11] & 1.63 & [1.37, 1.92] & 0.98 & [0.97, 0.98] \\ % fat real shortcut recon_sr data, but haven't had TotalSeg re-run on them yet.
& & Synth & 2.14 & [1.77, 2.50] & 7.49 & [6.22, 8.78] & 2.76 & [2.19, 3.38] & 0.92 & [0.86, 0.95] \\ %fat synth shortcut
& Weighted & Real & 1.58 & [1.08, 2.54] & 8.06 & [5.01, 13.67] & 1.80 & [1.77, 6.88]  & \multicolumn{2}{c}{---}\\
& OOD & Real & 3.79 & [3.13, 4.35] & 12.43 & [9.61, 16.60] & 4.68 & [3.82, 5.51] & 0.83 & [0.76, 0.88] \\
& & Recon & 3.93 & [3.38, 4.60] & 11.93 & [10.37, 13.72] & 4.71 & [4.03, 5.27] & 0.83 & [0.70, 0.88] \\ % fat real shortcut recon_sr data
& & Synth & 4.34 & [3.77, 4.97] & 13.97 & [12.01, 16.07] & 4.92 & [4.34, 5.61] & 0.79 & [0.69, 0.86]\\ %fat synth shortcut ood
\bottomrule
\end{tabular}
\label{tab:downstream}
\end{sidewaystable}


==> old_material/2024-11-22_tables.tex <==

% ctdownstream_eval split=bone_synth_old ckpt_path=...

% \begin{table}[h]
% \ra{1.3}
% \centering
% \caption{Validation on Downstream Tasks for Differently Biased Cohorts}
% \label{tab:shortcut-results}
% \begin{tabular}{@{}p{0.1em} l l rr rr rr@{}}
% \toprule
% \multicolumn{3}{@{}l}{\textbf{Downstream Task}} & \multicolumn{2}{c}{MAE} & \multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{RMSE}  \\
% \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
% & Sample & Source &\multicolumn{1}{l}{Value} & \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} \\
% \midrule
% \multicolumn{9}{@{}l}{\textbf{Muscle Percentage (\%)}} \\ % split on fat
% & IID & Real & 1.47 & [1.21, 1.80] & 4.45 & [3.64, 5.71] & 3.81 & [2.68, 6.54]\\
% && Recon & \\
% && Synth & 1.89 & [1.62, 2.26] & 5.75 & [4.86, 7.06] & 5.57 & [4.08, 8.51]\\
% & Weight & Real & \\
% & OOD & Real & 4.12 & [3.57, 4.71] & 19.05 & [16.14, 23.26] & 23.16 & [18.18, 30.61]\\
% && Recon & \\
% && Synth & 3.37 & [2.92, 3.88] & 14.35 & [12.11, 16.96] & 15.81 & [12.38, 20.39]\\
% \multicolumn{9}{@{}l}{\textbf{Body Fat Percentage (\%)}} \\ % split on muscle
% & IID & Real & 1.43 & [1.24, 1.67] & 5.69 & [4.78, 6.97] & 2.95 & [2.27, 4.29]\\
% && Recon & \\
% && Synth & 1.92 & [1.58, 2.32] & 7.57 & [6.05, 10.19] & 6.34 & [4.39, 9.02] \\
% & Weight & Real & \\
% & OOD & Real & 3.38 & [2.89, 3.95] & 11.62 & [9.30, 19.48] & 16.70 & [12.75, 22.86]\\
% && Recon & \\
% && Synth & 3.22 & [2.63, 3.96] & 9.73 & [8.21, 11.48] & 18.88 & [13.04, 27.08] \\
% \bottomrule
% \end{tabular}
% \label{tab:downstream}
% \end{table}


% \begin{sidewaystable}[h]
% \ra{1.3}
% \centering
% \caption{Validation on Downstream Tasks for Differently Biased Cohorts (Age Split)}
% \label{tab:performance_metrics}
% \begin{tabular}{@{}p{0.1em} l l rr rr rr rr@{}}
% \toprule
% \multicolumn{3}{@{}l}{\textbf{Downstream Task}} & \multicolumn{2}{c}{MAE} & \multicolumn{2}{c}{MAPE (\%)} & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{R\textsuperscript{2} Score} \\
% \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
% & Sample & Source &\multicolumn{1}{l}{Value} & \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value}& \multicolumn{1}{r}{CI} &\multicolumn{1}{l}{Value} &\multicolumn{1}{r}{CI} \\
% \midrule
% \multicolumn{3}{@{}l}{\textbf{Muscle Percentage (\%)}} & \multicolumn{8}{@{}l}{\textbf{80/20\% \wrt sex}}\\
% & Male & Real & 1.65 & [1.38, 1.94] & 5.33 & [4.33, 6.34] & 2.07 & [1.71, 2.41] & 0.82 & [0.72, 0.89] \\
% & & Synth & 1.30 & [1.08, 1.56] & 3.79 & [3.20, 4.47] & 1.64 & [1.34, 1.92] & 0.92 & [0.89, 0.95] \\
% & & Synth-rep & 1.62 & [1.36, 1.91] & 4.84 & [4.02, 5.58] & 1.95 & [1.74, 2.21] & 0.81 & [0.73, 0.87] \\
% & Female & Real & 1.85 & [1.51, 2.21] & 7.34 & [5.87, 8.80] & 2.32 & [1.92, 2.66] & 0.80 & [0.68, 0.86] \\
% & & Synth & 1.46 & [1.22, 1.73] & 5.02 & [4.07, 6.24] & 1.94 & [1.52, 2.36] & 0.90 & [0.83, 0.94] \\
% & & Synth-rep & 1.59 & [1.36, 1.83] & 5.46 & [4.64, 6.27] & 1.97 & [1.65, 2.25] & 0.86 & [0.80, 0.90] \\
% %
% \multicolumn{3}{@{}l}{\textbf{Body Fat Percentage (\%)}}& \multicolumn{8}{@{}l}{\textbf{80/20\% \wrt sex}} \\
% & Male & Real & 1.48 & [1.25, 1.71] & 5.73 & [4.80, 6.72] & 1.78 & [1.58, 2.01] & 0.96 & [0.94, 0.98] \\
% & & Synth & 1.98 & [1.62, 2.30] & 6.72 & [5.74, 7.96] & 2.46 & [2.01, 2.90] & 0.94 & [0.90, 0.96] \\
% & & Synth-rep & 1.81 & [1.58, 2.06] & 6.53 & [5.41, 7.62] & 2.15 & [1.95, 2.37] & 0.95 & [0.93, 0.97] \\
% & Female & Real & 1.95 & [1.61, 2.21] & 5.79 & [4.88, 6.59] & 2.36 & [2.00, 2.71] & 0.96 & [0.94, 0.97] \\
% & & Synth & 2.47 & [2.11, 3.00] & 7.63 & [6.42, 8.76] & 2.99 & [2.48, 3.38] & 0.93 & [0.88, 0.95]\\
% & & Synth-rep & 2.56 & [2.22, 2.97] & 8.13 & [6.70, 9.37] & 3.00 & [2.57, 3.34] & 0.93 & [0.90, 0.95] \\
% %
% \multicolumn{3}{@{}l}{\textbf{Bone Density (g/cm\textsuperscript{3})}} & \multicolumn{8}{@{}l}{\textbf{Normal dist.~\wrt age}} \\
% & Older & Real & 0.03 & [0.02, 0.03] & 1.78 & [1.44, 2.10] & 0.03 & [0.03, 0.04] & 0.76 & [0.65, 0.85] \\
% & & Synth & 0.04 & [0.04, 0.05] & 2.84 & [2.38, 3.31] & 0.05 & [0.04, 0.05] & -0.45 & [-1.07, 0.08] \\
% & Younger & Real & 0.02 & [0.02, 0.02] & 1.21 & [1.00, 1.43] & 0.02 & [0.02, 0.03] & 0.83 & [0.73, 0.89] \\
% & & Synth & 0.04 & [0.03, 0.04] & 2.50 & [2.16, 2.75] & 0.04 & [0.04, 0.05] & -0.65 & [-2.02, -0.01]\\
% \bottomrule
% \end{tabular}
% \label{tab:downstream}
% \end{sidewaystable}



==> old_material/2024-11-26_old-intro.tex <==
Abstract:
{
  Artificial intelligence (AI) is quickly becoming a cornerstone of modern radiology, accelerating triage,or offering second opinions to ensure correct medical image interpretation.
  However, the performance of AI models can degrade during clinical deployment due to population shifts, there is a need for population-specific clinical trials to ensure high performance for each adopting institution.
  However, deployment-time validation on collected imaging data is not practically feasible.
  Here we propose using conditional image synthesis as a flexible, scalable alternative to real data collection that can be incorporated much earlier in virtual clinical trials to anticipate changes in model performance on diverse target populations.
  We demonstrate for the first time that a generative model is capable of realistically synthesizing full-body, 3D computed tomography images, conditioned on patient attributes such as sex, age, height, and weight.
  Furthermore, we show in a controlled experiment that these images are of sufficient quality to replicate hidden biases in AI models that are otherwise present in real data.
  This method offers developers and regulatory bodies a scalable tool for identifying and correcting potential weaknesses in AI systems, ensuring their robustness across diverse populations over time.
  By enabling earlier detection of performance issues, our approach represents a significant advancement in ensuring the safety and efficacy of AI in healthcare.
}

Precision medicine aims to maximize healthcare quality by tailoring interventions to individuals.\cite{kosorok2019precision} % using data-driven decision-making
Central to this vision are algorithms developed using artificial intelligence and machine learning (AI/ML) to analyze medical images and support personalized, data-driven treatment plans. AI algorithms for automated CT analysis, for instance, have been used to assist in body composition measurement,\cite{zopfs2020evaluating} disease detection\cite{pickhardt2013opportunistic, jang2019opportunistic,eng2021automated, oh2024evaluation} and clinical decision-making.\cite{ozsahin2020review, murugesan2022a, mohammadi2024deep}
However, the performance of machine learning models may degrade during deployment due to population shift.\cite{oakden2020hidden, compton2023when, william2022external}
Anticipating performance degradations is paramount because an erroneous output can adversely affect patient outcomes and erode trust in AI systems.\cite{topol2019high}
Despite this, there is currently no way to ensure that the performance measured during pre-market development translates to post-market deployment.
While traditional clinical trials are appropriate for validating a model's initial performance through large scale cohort selection and data collection (see Fig.~\ref{fig:overview}a), they are not a practical solution for deployment-time validation due to cost and privacy considerations \cite{rajpurkar2022ai, menard2024artificial}.
% A single vendor may deploy an algorithm across thousands of client institutions.
At the same time, health care institutions are ill-equipped to validate AI systems on their own, due to lack of domain knowledge, computational resources, or sufficient access to proprietary models.
Thus, there is a need to replicate the gold standard or real clinical trials virtually, to evaluate model performance more easily and well in advance of deployments.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/overview.png}
    \caption{AI-based medical image analysis algorithms are susceptible to drops in performance when deployed on new populations. (a) The approval pipeline for medical image AI necessitates large cohort selection and costly data collection processes so as to ensure good performance across the given population. performance may still decline when deployed on new populations.\cite{oakden2020hidden}
      (b) We propose a novel framework for medical image AI validation, where a conditional generative model provides full-body images with the same distribution of attributes, \ie. demographics or other characteristics, as the target population. This enables \emph{in silico} clinical trials much earlier in the development pipeline, ensuring high performance on desired populations before real clinical trials.
      }
    \label{fig:overview}
\end{figure}

Central to this vision is the ability to synthesize medical images based on population-level attributes.
Current approaches relying on computational human phantoms\cite{abadi2020virtual, badano2023stochastic} are fundamentally limited in the types of variation they can express. These phantoms use boundary representations to capture variations in anatomical structures, making them well-suited for many types of virtual imaging trials\cite{segars2008realistic} but ultimately limited to shape-based variations.
It is not clear how to extend these phantoms to support population-level attributes.
Generative models using machine learning, on the other hand, are able to consume and produce practically unlimited data.\cite{ibrahim2024generative}
They have been used to improve model performance by augmenting training data with synthetic images.\cite{khader2023denoising}
In principle, generative models are highly flexible in the kind of conditioning parameters they can support, but there are significant challenges in developing a model with the capabilities necessary for conducting VCTs in precision medicine.

% ,\cite{bahrami2021comparison} anatomy,\cite{txurio2023diffusion, pan20232d} or conditioning parameters.\cite{guo2024maisi}

We demonstrate for the first time that a generative model is capable of realistically synthesizing full-body, 3D medical images. Furthermore, we show these images are of sufficient quality to replicate hidden biases in downstream models that are otherwise present in real data.
Rather than modeling the conditional distribution $p(\mathbf{X}|\mathbf{Y})$ of the 3D CT image $\mathbf{X}$ given an organ segmentation $\mathbf{Y}$,\cite{guo2024maisi} our approach ensures anatomical consistency by learning the joint distribution $p(\mathbf{X}, \mathbf{Y})$. This results in images that are visually and anatomically accurate, even compared to methods that focus on smaller regions and have access to detailed segmentations.
% as evaluated by quantitative similary measures and third-party segmentation algorithms.\cite{wasserthal2023totalsegmentator}
Our generative model achieves this consistency in a memory-efficient manner by operating on latent representations of the full-body image and segmentation.\cite{esser2020taming, rombach2022high}
We further model the distribution $p(\mathbf{X},\mathbf{Y}|\mathbf{a})$ conditioned on patient attributes $\mathbf{a}$, namely patient sex, age, height, and weight, to allow for sampling of virtual patient cohorts using a distribution of attributes.
These can be obtained from real health records of the deployment population or from statistical models, \eg, based on census data (see Fig.~\ref{fig:overview}b).
In controlled experiments, we show how virtual clinical trials (VCTs) using these cohorts can replicate model performance for multiple tasks in precision medicine, compared to performance on real data from the corresponding attribute distribution which would be otherwise inaccessible.
Whereas downstream models reliably estimate quantities like overall body fat and muscle mass percentage for data from the same attribute distribution as the training and validation data, those same models fail to generalize across a population shift because of hidden biases in the training data.
Those same degradations are observed on images generated from the synthetic patient cohort with the same attributes, which would enable a vendor to anticipate deployment time changes in performance and prevent adverse effects on patient care.




% Old paragraph 2, 2024-12-02
Degradations between controlled trial and deployment scenarios may result from differences, including the demographic makeup of the population, medical history, image collection protocols, and device specifications.
While clinical trials may detect such degradations through large scale cohort selection and data collection (see Fig.~\ref{fig:overview}a), they are not a practical solution for post-market deployment-time validation after significant investment in controlled trials \cite{rajpurkar2022ai, menard2024artificial}.
At the same time, health care institutions are ill-equipped to validate AI systems on their own, due to lack of domain knowledge, computational resources, or sufficient access to proprietary models.
Virtual Clinical Trials (VCTs), on the other hand, use \emph{in silico} simulation of medical images to replicate real world data collection processes.
\todo{Just want to say there are approaches for conducting virtual clinical trials, but there is no clear path to scaling these models.}
\todo{Current approaches relying on computational human phantoms\cite{abadi2020virtual, badano2023stochastic} are capable of representing differencing in imaging protocols and device specifications, but they are fundamentally limited in the types of variation they can express. Computational human phantoms use boundary representations to capture variations in anatomical structures, making them well-suited for many types of virtual imaging trials\cite{segars2008realistic} but ultimately limited to shape-based variations.
It is not clear how to extend these phantoms to examine a major likely cause for performance degradations between controlled trials and deployment populations, namely population-level patient attributes.}
Generative models using machine learning, on the other hand, are able to consume and produce practically unlimited data.\cite{ibrahim2024generative}
They have been used to improve model performance by augmenting training data with synthetic images.\cite{khader2023denoising}
In principle, generative models are highly flexible in the kind of conditioning parameters they can support, but there are significant challenges in developing a model with the capabilities necessary for conducting VCTs in precision medicine.

